Forecasting from LiDAR via Future Object Detection

Object detection and forecasting are fundamental components of embodied perception. These two problems, however, are largely studied in isolation by the community. In this paper, we propose an end-to-end approach for detection and motion forecasting based on raw sensor measurement as opposed to ground truth tracks. Instead of predicting the current frame locations and forecasting forward in time, we directly predict future object locations and backcast to determine where each trajectory began. Our approach not only improves overall accuracy compared to other modular or end-to-end baselines, it also prompts us to rethink the role of explicit tracking for embodied perception. Additionally, by linking future and current locations in a many-to-one manner, our approach is able to reason about multiple futures, a capability that was previously considered difficult for end-to-end approaches. We conduct extensive experiments on the popular nuScenes dataset and demonstrate the empirical effectiveness of our approach. In addition, we investigate the appropriateness of reusing standard forecasting metrics for an end-to-end setup, and find a number of limitations which allow us to build simple baselines to game these metrics. We address this issue with a novel set of joint forecasting and detection metrics that extend the commonly used AP metrics from the detection community to measuring forecasting accuracy. Our code is available at https://github.com/neeharperi/FutureDet

==> table/ablation_futuredet.tex <==
\begin{table*}[bt!]
\centering
   % \scriptsize
%   \setlength{\tabcolsep}{0.8pt}
   \setlength{\tabcolsep}{01.5pt}
      \resizebox{\linewidth}{!}{%
%\setlength{\tabcolsep}{1.5pt}
% \renewcommand{\arraystretch}{0.4}

\begin{tabular}{lccccccccccccccccccccccc}
\toprule 
 & \multicolumn{11}{c}{K=1} &  & \multicolumn{11}{c}{K=5}\tabularnewline
\cmidrule{2-12} \cmidrule{3-12} \cmidrule{4-12} \cmidrule{5-12} \cmidrule{6-12} \cmidrule{7-12} \cmidrule{8-12} \cmidrule{9-12} \cmidrule{10-12} \cmidrule{11-12} \cmidrule{12-12} \cmidrule{14-24} \cmidrule{15-24} \cmidrule{16-24} \cmidrule{17-24} \cmidrule{18-24} \cmidrule{19-24} \cmidrule{20-24} \cmidrule{21-24} \cmidrule{22-24} \cmidrule{23-24} \cmidrule{24-24} 
 & \multicolumn{2}{c}{$AP^{stat.}$} &  & \multicolumn{2}{c}{$AP^{lin.}$} &  & \multicolumn{2}{c}{$AP^{non-lin.}$} &  & \multicolumn{2}{c}{$mAP$} &  & \multicolumn{2}{c}{$AP^{stat.}$} &  & \multicolumn{2}{c}{$AP^{lin..}$} &  & \multicolumn{2}{c}{$AP^{non-lin.}$} &  & \multicolumn{2}{c}{$mAP$}\tabularnewline
\cmidrule{2-3} \cmidrule{3-3} \cmidrule{5-6} \cmidrule{6-6} \cmidrule{8-9} \cmidrule{9-9} \cmidrule{11-12} \cmidrule{12-12} \cmidrule{14-15} \cmidrule{15-15} \cmidrule{17-18} \cmidrule{18-18} \cmidrule{20-21} \cmidrule{21-21} \cmidrule{23-24} \cmidrule{24-24} 
 & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{mAP}_{\textrm{det.}}$ & $\textrm{mAP}_{\textrm{f}}$ &  & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{mAP}_{\textrm{det.}}$ & $\textrm{mAP}_{\textrm{f}}$\tabularnewline
\midrule 
% Detection + Constant Position (CP) & 62.0 & 54.0 & &  88.6 & 84.8  & & 3.6 & 0.0  & & 46.1 & 42.2  & & 62.0 & 54.0 & & 88.6 & 84.8 & & 3.6 & 0.0 & & 46.1 & 42.4  \tabularnewline
%\midrule 

\textbf{\futuredet}  & 70.1 & 65.5 &  & 62.9 & 24.9 &  & 91.8 & 10.1 &  & 74.9 & 33.5  &  & 0 & 0 &  & 0 & 0 &  & 0 & 0  &  & 0 & 0  \tabularnewline
w/o Recurrent Features  & 70.0 & 67.2 &  & 65.5 & 28.0 &  & 87.4 & 11.4  &  & 74.3 & 35.6  &  & 0 & 0 &  & 0 & 0 &  & 0 & 0  &  & 0 & 0 \tabularnewline
w/o Trajectory Sampler  & 69.5 & 65.2 &  & 64.8 & 24.9 &  & 89.1 & 7.8  &  & 74.4 & 32.6   &  & 0 & 0 &  & 0 & 0 &  & 0 & 0  &  & 0 & 0 \tabularnewline

% \midrule 
\bottomrule
\end{tabular}
}%


%
% Constant position (CP) &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
% \midrule 
% Constant velocity (CV) &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
% \midrule 
% Fast and Furious (FaF)~\cite{Luo18CVPR}. &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
% %
% Our+precast (post NMS) &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
% \midrule 
% Our+precast (pre NMS) &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
% \midrule 
% Our + bi-directional &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
% \midrule 
% Our+conditioned &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline


\caption{We study the impact of architectural and training modifications to \futuredet. We find that adding recurrent features and trajectory sampling primarily improves $AP_f^{non-lin.}$. Moreover, we see the \futuredet improves $mAP_f$ considerably at $K=5$} %\deva{We don't define base AP. Should we just remove the firsrt 2 cols?}} 
\label{tab:ablation_recurrent}
\end{table*}

% Constant position (CP).
% Constant velocity (CV).
% Fast and Furious (FaF)~\cite{Luo18CVPR}.
% } 
% Our+precast+post-NMS:} 
% Our+bi-directional:} 
% Our+conditioned:}

==> table/ade_table.tex <==
\begin{table}[t]
\centering{}
\scriptsize
\setlength{\tabcolsep}{1.5pt}

\begin{tabular}{lccccc}
\toprule 
 & \multicolumn{2}{c}{ADE \textdownarrow{}} &  & \multicolumn{2}{c}{FDE \textdownarrow{}}\tabularnewline
\cmidrule{2-3} \cmidrule{3-3} \cmidrule{5-6} \cmidrule{6-6} 
 & 60\% TP & 90\% TP &  & 60\% TP & 90\% TP\tabularnewline
\midrule 
PnP & 0.58 & 0.68 &  & 0.93 & 1.04\tabularnewline
\midrule 
FutureDet. + Backcast &  0.37 &   &  & 0.56 & \tabularnewline
\midrule 
FutureDet. + Backcast + Match & 0.73 &  &  &  & \tabularnewline
\bottomrule
\end{tabular}

\caption{Table of ADE results.}
\label{table:ade}
\end{table}


% \begin{table}[t]
% \centering{}
% \scriptsize
% \setlength{\tabcolsep}{1.5pt}

% COPY TEXT FROM LYX HERE

% \caption{Table of ADE results.}
% \label{table:ade}
% \end{table}

==> table/jitter.tex <==
\begin{table}[t]
\centering
   % \scriptsize
%   \setlength{\tabcolsep}{0.8pt}
   \setlength{\tabcolsep}{01.5pt}
      \resizebox{\linewidth}{!}{%
%\setlength{\tabcolsep}{1.5pt}
% \renewcommand{\arraystretch}{0.4}

\begin{tabular}{lccccccccccc}
\toprule 
 & \multicolumn{11}{c}{K=5}\tabularnewline
\cmidrule{2-12}
 & \multicolumn{2}{c}{$AP$} &  & \multicolumn{2}{c}{$AP^{stat.}$} &  & \multicolumn{2}{c}{$AP^{mov.}$} &  & \multicolumn{2}{c}{$mAP$}\tabularnewline
\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12}
 & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{mAP}_{\textrm{det.}}$ & $\textrm{mAP}_{\textrm{f}}$\tabularnewline
\midrule 
% Detection + Constant Position (CP) & 62.0 & 54.0 & &  88.6 & 84.8  & & 3.6 & 0.0  & & 46.1 & 42.2  & & 62.0 & 54.0 & & 88.6 & 84.8 & & 3.6 & 0.0 & & 46.1 & 42.4  \tabularnewline
%\midrule 
Detection + Constant Velocity & \textbf{83.9} & 52.6 & & \textbf{90.0} & 84.2 & & \textbf{91.4} & 11.7 & & \textbf{90.7}  & 47.9 \tabularnewline

Detection + Constant Velocity w/ Jitter & \textbf{83.9} & 56.6 & & \textbf{90.0} & 85.0 & & \textbf{91.4} & 18.7 & & \textbf{90.7}  & 51.9 \tabularnewline
%\midrule 
Detection + Forecast (\cf~\cite{Luo18CVPR}) & 82.4 & 51.3 & & 89.1 & 83.5 & & 90.3 & 10.7 & & 89.7  & 47.1 \tabularnewline

Detection + Forecast w/ Jitter (\cf~\cite{Luo18CVPR}) & 82.4 & 55.0 & & 89.1 & 84.8 & & 90.3 & 17.3 & & 89.7  & 51.1 \tabularnewline
%\midrule

Trajectron++~\cite{salzmann2020eccv}  & 83.5 & 46.6 &  & 88.9 & 79.2 &  & 88.6 & 7.4  &  & 88.8 & 43.3\tabularnewline

\rowcolor{green!10} \textbf{FutureDet + Backcast + Match}  & 81.2 & 57.2 &  &  89.2 & 84.9  &  & 89.4 & \textbf{20.0} & & 89.3 & \textbf{52.5} \tabularnewline
% \midrule 
\bottomrule
\end{tabular}
}%


%
% Constant position (CP) &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
% \midrule 
% Constant velocity (CV) &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
% \midrule 
% Fast and Furious (FaF)~\cite{Luo18CVPR}. &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
% %
% Our+precast (post NMS) &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
% \midrule 
% Our+precast (pre NMS) &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
% \midrule 
% Our + bi-directional &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
% \midrule 
% Our+conditioned &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline


\caption{We augment single-future baselines by sampling five new trajectories from a Gaussian distribution. We generate new trajectories by sampling velocity estimates derived from the predicted velocity. Each sampled velocity has mean $v_p$, and standard deviation of $||v_p||$. This simple augmentation significantly improves trajectory forecasting for single-future baselines at K=5, but does not beat \futuredet.}
\label{table:jitter_results}
\end{table}

% Constant position (CP).
% Constant velocity (CV).
% Fast and Furious (FaF)~\cite{Luo18CVPR}.
% } 
% Our+precast+post-NMS:} 
% Our+bi-directional:} 
% Our+conditioned:}

==> table/jitter_backup.tex <==
\begin{table*}[t]
\centering
   % \scriptsize
%   \setlength{\tabcolsep}{0.8pt}
   \setlength{\tabcolsep}{01.5pt}
      \resizebox{\linewidth}{!}{%
%\setlength{\tabcolsep}{1.5pt}
% \renewcommand{\arraystretch}{0.4}

\begin{tabular}{lccccccccccccccccccccccc}
\toprule 
 & \multicolumn{11}{c}{K=1} &  & \multicolumn{11}{c}{K=5}\tabularnewline
\cmidrule{2-12} \cmidrule{3-12} \cmidrule{4-12} \cmidrule{5-12} \cmidrule{6-12} \cmidrule{7-12} \cmidrule{8-12} \cmidrule{9-12} \cmidrule{10-12} \cmidrule{11-12} \cmidrule{12-12} \cmidrule{14-24} \cmidrule{15-24} \cmidrule{16-24} \cmidrule{17-24} \cmidrule{18-24} \cmidrule{19-24} \cmidrule{20-24} \cmidrule{21-24} \cmidrule{22-24} \cmidrule{23-24} \cmidrule{24-24} 
 & \multicolumn{2}{c}{$AP$} &  & \multicolumn{2}{c}{$AP^{stat.}$} &  & \multicolumn{2}{c}{$AP^{mov.}$} &  & \multicolumn{2}{c}{$mAP$} &  & \multicolumn{2}{c}{$AP$} &  & \multicolumn{2}{c}{$AP^{stat.}$} &  & \multicolumn{2}{c}{$AP^{mov.}$} &  & \multicolumn{2}{c}{$mAP$}\tabularnewline
\cmidrule{2-3} \cmidrule{3-3} \cmidrule{5-6} \cmidrule{6-6} \cmidrule{8-9} \cmidrule{9-9} \cmidrule{11-12} \cmidrule{12-12} \cmidrule{14-15} \cmidrule{15-15} \cmidrule{17-18} \cmidrule{18-18} \cmidrule{20-21} \cmidrule{21-21} \cmidrule{23-24} \cmidrule{24-24} 
 & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{mAP}_{\textrm{det.}}$ & $\textrm{mAP}_{\textrm{f}}$\tabularnewline
\midrule 
% Detection + Constant Position (CP) & 62.0 & 54.0 & &  88.6 & 84.8  & & 3.6 & 0.0  & & 46.1 & 42.2  & & 62.0 & 54.0 & & 88.6 & 84.8 & & 3.6 & 0.0 & & 46.1 & 42.4  \tabularnewline
%\midrule 
Detection + Constant Velocity & \textbf{83.9} & 52.6 &  & \textbf{90.0} & 84.2 & & \textbf{91.4} & 11.7 & & \textbf{90.7}  & 47.95 &  & \textbf{83.9} & 52.6 & & \textbf{90.0} & 84.2 & & \textbf{91.4} & 11.7 & & \textbf{90.7}  & 47.9 \tabularnewline

Detection + Constant Velocity w/ Jitter & \textbf{83.9} & 52.6 &  & \textbf{90.0} & 84.2 & & \textbf{91.4} & 11.7 & & \textbf{90.7}  & 47.95 &  & \textbf{83.9} & 56.6 & & \textbf{90.0} & 85.0 & & \textbf{91.4} & 18.7 & & \textbf{90.7}  & 51.9 \tabularnewline
%\midrule 
Detection + Forecast (\cf~\cite{Luo18CVPR}) & 82.4 & 51.3 & & 89.1 & 83.5 & & 90.3 & 10.7 & & 89.7 & 47.1 & & 82.4 & 51.3 & & 89.1 & 83.5 & & 90.3 & 10.7 & & 89.7  & 47.1 \tabularnewline

Detection + Forecast w/ Jitter (\cf~\cite{Luo18CVPR}) & 82.4 & 51.3 & & 89.1 & 83.5 & & 90.3 & 10.7 & & 89.7 & 47.1 & & 82.4 & 55.0 & & 89.1 & 84.8 & & 90.3 & 17.3 & & 89.7  & 51.1 \tabularnewline
%\midrule

Trajectron++~\cite{salzmann2020eccv}  & 83.5 & 44.2 &  & 88.9 & 77.7 &  & 88.6 & 3.2 &  & 88.8 & 40.45  &  & 83.5 & 46.6 &  & 88.9 & 79.2 &  & 88.6 & 7.4  &  & 88.8 & 43.3\tabularnewline

\rowcolor{green!10} \textbf{FutureDet + Backcast + Match}  & 81.2 & 54.7 &  & 89.2 & 84.8 & & 89.4 & \textbf{16.0} &  & 89.3 & \textbf{50.4} & & 81.2 & 57.2 &  &  89.2 & 84.9  &  & 89.4 & \textbf{20.0} & & 89.3 & \textbf{52.5} \tabularnewline
% \midrule 
\bottomrule
\end{tabular}
}%


%
% Constant position (CP) &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
% \midrule 
% Constant velocity (CV) &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
% \midrule 
% Fast and Furious (FaF)~\cite{Luo18CVPR}. &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
% %
% Our+precast (post NMS) &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
% \midrule 
% Our+precast (pre NMS) &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
% \midrule 
% Our + bi-directional &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
% \midrule 
% Our+conditioned &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline


\caption{We augment single-future baselines by sampling five new trajectories from a Gaussian distribution. We generate new trajectories by sampling velocity estimates derived from the predicted velocity. Each sampled velocity has mean $v_p$, and standard deviation of $||v_p||$. This simple augmentation significantly improves trajectory forecasting for single-future baselines at K=5, but does not beat \futuredet.}
\label{table:jitter_results}
\end{table*}

% Constant position (CP).
% Constant velocity (CV).
% Fast and Furious (FaF)~\cite{Luo18CVPR}.
% } 
% Our+precast+post-NMS:} 
% Our+bi-directional:} 
% Our+conditioned:}

==> table/rebut_tab.tex <==
\begin{table*}[t!]
\centering
   \scriptsize
%   \setlength{\tabcolsep}{0.8pt}
   \setlength{\tabcolsep}{01.5pt}
   %\resizebox{\linewidth}{!}{%
%\setlength{\tabcolsep}{1.5pt}
% \renewcommand{\arraystretch}{0.4}
\begin{tabular}{lccccccccccccccccccccccc}
\toprule 
 & \multicolumn{11}{c}{K=1} &  & \multicolumn{11}{c}{K=5}\tabularnewline
\cmidrule{2-12} \cmidrule{3-12} \cmidrule{4-12} \cmidrule{5-12} \cmidrule{6-12} \cmidrule{7-12} \cmidrule{8-12} \cmidrule{9-12} \cmidrule{10-12} \cmidrule{11-12} \cmidrule{12-12} \cmidrule{14-24} \cmidrule{15-24} \cmidrule{16-24} \cmidrule{17-24} \cmidrule{18-24} \cmidrule{19-24}  \cmidrule{20-24} \cmidrule{21-24} \cmidrule{22-24} \cmidrule{23-24} \cmidrule{24-24} 
 & \multicolumn{2}{c}{$AP^{stat.}$} &  & \multicolumn{2}{c}{$AP^{lin.}$} &  & \multicolumn{2}{c}{$AP^{nonlin.}$} &  & \multicolumn{2}{c}{$mAP$} &  & \multicolumn{2}{c}{$AP^{stat.}$} &  & \multicolumn{2}{c}{$AP^{lin.}$} &  & \multicolumn{2}{c}{$AP^{nonlin.}$} &  & \multicolumn{2}{c}{$mAP$}\tabularnewline
\cmidrule{2-3} \cmidrule{3-3} \cmidrule{5-6} \cmidrule{6-6} \cmidrule{8-9} \cmidrule{9-9} \cmidrule{11-12} \cmidrule{12-12} \cmidrule{14-15} \cmidrule{15-15} \cmidrule{17-18} \cmidrule{18-18} \cmidrule{20-21} \cmidrule{21-21} \cmidrule{23-24} \cmidrule{24-24} 
 & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{AP}_{\textrm{det.}}$ & $\textrm{AP}_{\textrm{f}}$ &  & $\textrm{mAP}_{\textrm{det.}}$ & $\textrm{mAP}_{\textrm{f}}$\tabularnewline
\midrule 
% Detection + Constant Position (CP) & 62.0 & 54.0 & &  88.6 & 84.8  & & 3.6 & 0.0  & & 46.1 & 42.2  & & 62.0 & 54.0 & & 88.6 & 84.8 & & 3.6 & 0.0 & & 46.1 & 42.4  \tabularnewline
%\midrule 
Det. + CV & 91.1 & 85.9 &  & 91.9 & 28.5 & & 89.2 & 5.3 & & 90.7  & 39.9 &  & 91.1 & 85.9 &  & 91.9 & 28.5 & & 89.2 & 5.3 & & 90.7  & 39.9 \tabularnewline
%\midrule 
%\midrule
FaF*  & 88.1 & 81.1 &  & 90.0 & 31.5 & & 88.8 & 10.2 & & 89.0  & 40.9 &  & 88.1 & 81.1 &  & 90.0 & 31.5 & & 88.8 & 10.2 & & 89.0  & 40.9 \tabularnewline
%
Traj.++  & 0 & 0 &  & 0 & 0 & & 0 & 0 & & 0  & 0 &  & 0 & 0 & & 0 & 0 & & 0 & 0 & & 0  & 0 \tabularnewline
%
DenseTNT  & 0 & 0 &  & 0 & 0 & & 0 & 0 & & 0  & 0 &  & 0 & 0 & & 0 & 0 & & 0 & 0 & & 0  & 0 \tabularnewline
%
\midrule 
%\midrule 
\textbf{FutDet}  & 92.2 & 85.7 &  & 92.5 & 27.5 & & 91.7 & 13.3 & & 92.1  & 42.2 &  & 92.2 & 88.8 & & 92.5 & 45.8 & & 91.7 & 25.1 & & 92.1  & 53.3 \tabularnewline
%
\textbf{FutDet-PP}  & 0 & 0 &  & 0 & 0 & & 0 & 0 & & 0  & 0 &  & 0 & 0 & & 0 & 0 & & 0 & 0 & & 0  & 0 \tabularnewline
%
\textbf{FutDet w/ Map} & 0 & 0 &  & 0 & 0 & & 0 & 0 & & 0  & 0 &  & 0 & 0 & & 0 & 0 & & 0 & 0 & & 0  & 0 \tabularnewline

% \midrule 
\bottomrule
\end{tabular}
%}%
%
\caption{TODO}
\label{table:results}
\end{table*}


% Constant position (CP).
% Constant velocity (CV).
% Fast and Furious (FaF)~\cite{Luo18CVPR}.
% } 
% Our+precast+post-NMS:} 
% Our+bi-directional:} 
% Our+conditioned:}

==> table/rebut_tab_aljosa.tex <==
\begin{table}[t!]
\centering
   \tiny
%   \setlength{\tabcolsep}{0.8pt}
   \setlength{\tabcolsep}{01.5pt}
   %\resizebox{\linewidth}{!}{%
%\setlength{\tabcolsep}{1.5pt}
% \renewcommand{\arraystretch}{0.4}



\begin{tabular}{cclccccccccccc}
\toprule 
 &  &  & \multicolumn{2}{c}{$\textrm{AP}^{\textrm{stat.}}$} &  & \multicolumn{2}{c}{$\textrm{AP}^{\textrm{lin.}}$} &  & \multicolumn{2}{c}{$\textrm{AP}^{\textrm{nonlin.}}$} &  & \multicolumn{2}{c}{$\textrm{mAP}$}\tabularnewline
\cmidrule{4-5} \cmidrule{7-8}  \cmidrule{10-11} \cmidrule{13-14} 
 & \# &  & $\textrm{AP}_{\textrm{det.}}$  & $\textrm{AP}_{\textrm{f}}$  &  & $\textrm{AP}_{\textrm{det.}}$  & $\textrm{AP}_{\textrm{f}}$  &  & $\textrm{AP}_{\textrm{det.}}$  & $\textrm{AP}_{\textrm{f}}$  &  & $\textrm{mAP}_{\textrm{det.}}$  & $\textrm{mAP}_{\textrm{f}}$\tabularnewline
\midrule 
\parbox[t]{3mm}{%
\multirow{7}{*}{\rotatebox[origin=c]{90}{Cars}}%
}  & 1 & Det. + CV  & 91.1  & 85.9  &  & 91.9  & 28.5  &  & 89.2  & 5.3  &  & 90.7  & 39.9 \tabularnewline
 & 2 & FaF{*}  & 90.8  & 85.3  &  & 91.1  & 29.4  &  & 89.7  & 6.6  &  & 90.6  & 40.4 \tabularnewline
 & 3 & Traj.++  & 91.1  & 78.3  &  & 91.9  & 9.1  &  & 89.2  & 7.0  &  & 90.7  & 31.5 \tabularnewline
\cmidrule{2-14} 
%  & 4 & \textbf{FutDet-noResamp.}  & 91.1  & 87.2  &  & 91.4  & 32.2  &  & 89.4  & 7.4  &  & 0  & 0 \tabularnewline
 & 4 & \textbf{FutDet}  & 92.2  & 87.6  &  & 92.5  & 32.5  &  & 91.7  & 10.7  &  & 92.1  & 43.6 \tabularnewline
 & 5 & \textbf{FutDet-PP}  & \textbf{93.1}  & 87.4  &  & \textbf{92.8}  & \textbf{33.3}  &  & \textbf{91.9}  & \textbf{12.1}  &  & \textbf{92.6}  & \textbf{44.3} \tabularnewline
 & 6 & \textbf{FutDet w/ Map}  & 92.2  & \textbf{87.7}  &  & 92.5  & 31.8  &  & 91.1  & 10.7  &  & 91.9  & 43.4 \tabularnewline
\midrule 
\parbox[t]{3mm}{%
\multirow{7}{*}{\rotatebox[origin=c]{90}{Pedestrians}}%
}  & 7 & Det. + CV  & 95.0  & 57.5  &  & 98.1  & 36.7  &  & 96.9  & 12.8  &  & 96.7  & 35.7 \tabularnewline
 & 8 & FaF{*}  & 95.0  & 61.7  &  & 98.3  & \textbf{40.5}  &  & 97.2  & 13.8  &  & 96.9  & \textbf{38.7} \tabularnewline
 & 9 & Traj.++  & 95.0  & 31.8  &  & 98.1  & 10.9  &  & 96.9  & 8.6  &  & 96.7  & 17.1 \tabularnewline
\cmidrule{2-14} 
 & 10 & \textbf{FutDet}  & \textbf{95.8}  & \textbf{63.1}  &  & 98.1  & 37.2  &  & \textbf{97.8}  & 14.3  &  & \textbf{97.3}  & 38.2 \tabularnewline
 & 11 & \textbf{FutDet-PP}  & 93.6  & 54.5  &  & \textbf{98.6}  & 33.9  &  & \textbf{97.8}  &  12.5 &  & 96.6  & 33.6 \tabularnewline
 & 12 & \textbf{FutDet w/ Map}  & \textbf{95.8}  & 62.8  &  & 98.1  & 37.0  &  & 97.5  & \textbf{15.0}  &  & 97.1  & 38.3 \tabularnewline
\bottomrule
\end{tabular}


%}%
%
\vspace{-5pt}
\caption{Results for K=1. FutDet variants improve over baselines for both cars and pedestrians on the nuScenes dataset.}
\label{table:results}
\end{table}


% Constant position (CP).
% Constant velocity (CV).
% Fast and Furious (FaF)~\cite{Luo18CVPR}.
% } 
% Our+precast+post-NMS:} 
% Our+bi-directional:} 
% Our+conditioned:}

==> table/trajectron_table.tex <==
\begin{table*}[t]
\centering{}
\scriptsize
\setlength{\tabcolsep}{1.5pt}

\begin{tabular}{lcccccccccccccccccccccccc}
\toprule 
 &  & \multicolumn{11}{c}{Car} &  & \multicolumn{11}{c}{Pedestrian}\tabularnewline
\cmidrule{3-13} \cmidrule{4-13} \cmidrule{5-13} \cmidrule{6-13} \cmidrule{7-13} \cmidrule{8-13} \cmidrule{9-13} \cmidrule{10-13} \cmidrule{11-13} \cmidrule{12-13} \cmidrule{13-13} \cmidrule{15-25} \cmidrule{16-25} \cmidrule{17-25} \cmidrule{18-25} \cmidrule{19-25} \cmidrule{20-25} \cmidrule{21-25} \cmidrule{22-25} \cmidrule{23-25} \cmidrule{24-25} \cmidrule{25-25} 
 &  & \multicolumn{2}{c}{All} &  & \multicolumn{2}{c}{Static} &  & \multicolumn{2}{c}{Dynamic} &  & \multicolumn{2}{c}{Balanced} &  & \multicolumn{2}{c}{All} &  & \multicolumn{2}{c}{Static} &  & \multicolumn{2}{c}{Dynamic} &  & \multicolumn{2}{c}{Balanced}\tabularnewline
\cmidrule{3-4} \cmidrule{4-4} \cmidrule{6-7} \cmidrule{7-7} \cmidrule{9-10} \cmidrule{10-10} \cmidrule{12-13} \cmidrule{13-13} \cmidrule{15-16} \cmidrule{16-16} \cmidrule{18-19} \cmidrule{19-19} \cmidrule{21-22} \cmidrule{22-22} \cmidrule{24-25} \cmidrule{25-25} 
 & Maps & $\textrm{AP}_{\textrm{D}}$ & $\textrm{AP}_{\textrm{F}}$ &  & $\textrm{AP}_{\textrm{D}}$ & $\textrm{AP}_{\textrm{F}}$ &  & $\textrm{AP}_{\textrm{D}}$ & $\textrm{AP}_{\textrm{F}}$ &  & $\textrm{AP}_{\textrm{D}}$ & $\textrm{AP}_{\textrm{F}}$ &  & $\textrm{AP}_{\textrm{D}}$ & $\textrm{AP}_{\textrm{F}}$ &  & $\textrm{AP}_{\textrm{D}}$ & $\textrm{AP}_{\textrm{F}}$ &  & $\textrm{AP}_{\textrm{D}}$ & $\textrm{AP}_{\textrm{F}}$ &  & $\textrm{AP}_{\textrm{D}}$ & $\textrm{AP}_{\textrm{F}}$\tabularnewline
\midrule 
\multirow{2}{*}{Trajectron++ (with GT dets + tracks)} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
\cmidrule{2-25} \cmidrule{3-25} \cmidrule{4-25} \cmidrule{5-25} \cmidrule{6-25} \cmidrule{7-25} \cmidrule{8-25} \cmidrule{9-25} \cmidrule{10-25} \cmidrule{11-25} \cmidrule{12-25} \cmidrule{13-25} \cmidrule{14-25} \cmidrule{15-25} \cmidrule{16-25} \cmidrule{17-25} \cmidrule{18-25} \cmidrule{19-25} \cmidrule{20-25} \cmidrule{21-25} \cmidrule{22-25} \cmidrule{23-25} \cmidrule{24-25} \cmidrule{25-25} 
 & \xmark &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
\midrule 
\multirow{2}{*}{Trajectron++ (with predicted dets + tracks)} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
\cmidrule{2-25} \cmidrule{3-25} \cmidrule{4-25} \cmidrule{5-25} \cmidrule{6-25} \cmidrule{7-25} \cmidrule{8-25} \cmidrule{9-25} \cmidrule{10-25} \cmidrule{11-25} \cmidrule{12-25} \cmidrule{13-25} \cmidrule{14-25} \cmidrule{15-25} \cmidrule{16-25} \cmidrule{17-25} \cmidrule{18-25} \cmidrule{19-25} \cmidrule{20-25} \cmidrule{21-25} \cmidrule{22-25} \cmidrule{23-25} \cmidrule{24-25} \cmidrule{25-25} 
 & \xmark &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
\midrule 
Ours &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
\bottomrule
\end{tabular}


\caption{Table of results with comparison to non-end-to-end methods.}
\label{table:traj}
\end{table*}
